Enriques involutions on pencils of K3 surfaces

The three pencils of K3 surfaces of minimal discriminant whose general element covers at least one Enriques surface are Kond\={o}'s pencils I and II, and the Ap\'ery--Fermi pencil. We enumerate and investigate all Enriques surfaces covered by their general elements.

==> tables/genus_Barth_Peters.tex <==
\begin{table}[t]
    \centering
    \caption{Lattices in the frame genus \(\cW_X\) of a K3 surface \(X\) with transcendental lattice \(T_X \cong \bU \oplus \bU(2)\).}
    \label{tab:genus_Barth_Peters}
    \begin{tabular}{lllllll}
    \toprule 
    \(W\) & \(W_\rootlattice\) & \(W/W_\rootlattice\) & \(|\Delta(W)|\) & \(|{\OO(W)}|\) & \(|{\fr_X^{-1}(W)}|\) \\
    \midrule
    \(W_1\) & \(\bD_8\bE_8\) & \(0\)                    & \(352\) & \(7191587192832000\)    & \(1\) \\
    \(W_2\) & \(\bD_{16}\)  & \(0\)                     & \(480\) & \(1371195958099968000\) & \(1\) \\
    \midrule 
    \(W_3\) & \(\bD_8^2\)   & \(\IZ/2\IZ\)              & \(224\) & \(53271016243200\)      & \(2\) \\
    \(W_4\) & \(\bA_1^2\bE_7^2\) & \(\IZ/2\IZ\)         & \(256\) & \(134842259865600\)     & \(1\) \\
    \(W_5\) & \(\bD_4 \bD_{12}\) & \(\IZ/2\IZ\)         & \(288\) & \(376702186291200\)     & \(1\) \\
    \midrule
    \(W_6\) & \(\bA_{15}\)  & \(\IZ \oplus (\IZ/2\IZ)\) & \(240\) & \(83691159552000\)      & \(1\) \\
    \bottomrule
    \end{tabular}
\end{table}
